Memory Mosaics

Memory Mosaics are networks of associative memories working in concert to achieve a prediction task of interest. Like transformers, memory mosaics possess compositional capabilities and in-context learning capabilities. Unlike transformers, memory mosaics achieve these capabilities in comparatively transparent way ("predictive disentanglement"). We illustrate these capabilities on a toy example and also show that memory mosaics perform as well or better than transformers on medium-scale language modeling tasks.

==> images/clipart/fixpdf <==
#!/bin/sh 

for i
do
    r=`dirname "$i"`/`basename "$i" ".pdf"`
    pdftops $i $r.ps \
        && ( rm 2>/dev/null $r.eps ; ps2eps -l -H $r.ps ) \
        && ( ps2pdf14 -dEPSCrop $r.eps $i )
    rm 2>/dev/null $r.ps
done



